Know Your Needs Better: Towards Structured Understanding of Marketer Demands with Analogical Reasoning Augmented LLMs

In this paper, we explore a new way for user targeting, where non-expert marketers could select their target users solely given demands in natural language form. The key to this issue is how to transform natural languages into practical structured logical languages, i.e., the structured understanding of marketer demands. In practical scenarios, the demands of non-expert marketers are often abstract and diverse. Considering the impressive natural language processing ability of large language models (LLMs), we try to leverage LLMs to solve this issue. To stimulate the LLMs' reasoning ability, the chain-of-thought (CoT) prompting method is widely used, but existing methods still have some limitations in our scenario: (1) Previous methods either use simple "Let's think step by step" spells or provide fixed examples in demonstrations without considering compatibility between prompts and concrete questions, making LLMs ineffective when the marketers' demands are abstract and diverse. (2) Previous methods are often implemented in closed-source models or excessively large models, which is not suitable in industrial practical scenarios. Based on these, we propose ARALLM (i.e., Analogical Reasoning Augmented Large Language Models) consisting of two modules: Analogical Reasoning based Prompting and Reasoning-Augmented Multi-Task Model Distillation. Part of our data and code can be found at https://github.com/alipay/Analogic-Reasoning-Augmented-Large-Language-Model.

==> table/case_study.tex <==
\begin{table}[t]
    \centering
    \caption{Case study on ChatGPT with different versions of prompt. Bad responses are marked with a wavy underline.}
    % \vspace{-3mm}
    % \small
    \begin{tabularx}{0.5\textwidth}{l|X}
    
    \toprule
     \rowcolor{light-gray}\multicolumn{2}{c}{Demand:\textit{Company white-collar workers who enjoy drinking Starbucks}} 
     \\
      \hline
      Zero-shot &  {(Preference\#Belongs To\#Starbucks)}\\
      \hline
      Fixed few-shot  &  {(Preference\#Belongs To\#Starbucks) AND (Resident City\#Belongs To\#\uwave{Company white-collar)}}\\
      \hline
      Fixed few-shot + RS  &  {(Preference\#Belongs To\#\uwave{Enjoy} drinking Starbucks) AND (Resident City\#Belongs To\#\uwave{Company white-collar})} \\
      \hline
      Random few-shot + RS &  {(Preference\#Belongs To\#Starbucks)}\\
      \hline
      ARAP & \textbf{(Preference\#Belongs To\#Starbucks) AND (Career\#Belongs To\#White-collar)} \\
    \midrule
    \rowcolor{light-gray}\multicolumn{2}{c}{Demand:\textit{Young men who enjoy collecting toy models}} 
     \\
      \hline
      Zero-shot &  {(Preference\#\uwave{Contain}\#Toy models) AND (Gender\#\uwave{Equal To}\#Male) AND (Age\#\uwave{Belongs To}\#\uwave{[18,30]})}\\
      \hline
      Fixed few-shot  &  {(Preference\#Belongs To\#Toy models) AND (Gender\#Belongs To\#Male) AND (Age\uwave{\#Less Than\#30})}\\
      \hline
      Fixed few-shot + RS &   {(Preference\#Belongs To\#Toy models) AND (Gender\#Belongs To\#Male)} \\
      \hline
      Random few-shot + RS &  {(Preference\#Belongs To\#Toy models) AND (Gender\#Belongs To\#Male) AND (Age\#Belongs To\#\uwave{Young})}\\
      \hline
      ARAP &  \textbf{(Preference\#Belongs To\#Toy models) AND (Gender\#Belongs To\#Male) AND (Age\#Between\#18,35)} \\
    \bottomrule
    \end{tabularx}

    \label{tab:case_study}
\end{table}
